Node-wise Filtering in Graph Neural Networks: A Mixture of Experts Approach

Graph Neural Networks (GNNs) have proven to be highly effective for node classification tasks across diverse graph structural patterns. Traditionally, GNNs employ a uniform global filter, typically a low-pass filter for homophilic graphs and a high-pass filter for heterophilic graphs. However, real-world graphs often exhibit a complex mix of homophilic and heterophilic patterns, rendering a single global filter approach suboptimal. In this work, we theoretically demonstrate that a global filter optimized for one pattern can adversely affect performance on nodes with differing patterns. To address this, we introduce a novel GNN framework Node-MoE that utilizes a mixture of experts to adaptively select the appropriate filters for different nodes. Extensive experiments demonstrate the effectiveness of Node-MoE on both homophilic and heterophilic graphs.

==> theory.tex <==
\section{Proof}

Let $\left(\varepsilon_k\right)_{k \in[n]}$ be i.i.d. $\operatorname{Ber}\left(\frac{1}{2}\right)$ random variables. There are two classes $C_0=\left\{i \in[n]: \varepsilon_i=0\right\}$ and $C_1=C_0^c$. For each node, consider $\vX \in \RR^{n \times d}$ to be the feature matrix such that each row $\vX_i$ is an independent $d$-dimensional Gaussian random vectors with $X_i \sim N\left(\boldsymbol{\mu}, \frac{1}{d} \vI\right)$ if $i \in C_0$ and $X_i \sim N\left(\boldsymbol{\nu}, \frac{1}{d} \vI\right)$ if $i \in C_1$. Here $\boldsymbol{\mu}, \boldsymbol{\nu}$ are the fixed class mean vector with $\|\boldsymbol{\mu}\|_2,\|\boldsymbol{\nu}\|_2 \leq 1$ and $\vI$ is the identity matrix. Suppose there are two patterns of nodes in the adjacency matrix $\vA=(a_{ij})$, the homophilic pattern: 
$H_0 = \{i \in[n]: a_{ij} = \operatorname{Ber}(p_0)$ \text{if} $\varepsilon_i = \varepsilon_j $ and
$a_{ij} = \operatorname{Ber}(q_0)$ if $\varepsilon_i \neq \varepsilon_j , p_0 > q_0 \}$ and the heterophilic pattern: $H_1 = \{i \in[n]: a_{ij} = \operatorname{Ber}(p_1)$ \text{if} $\varepsilon_i = \varepsilon_j $ and
$a_{ij} = \operatorname{Ber}(q_1)$ if $\varepsilon_i \neq \varepsilon_j , p_1 < q_1 \}$.

$m(i)=\mathbb{E}\left[\tilde{X}_i \mid A, \varepsilon\right]=\frac{1}{D_{i i}} \sum_{j \in[n]} \tilde{a}_{i j} \vX_j .$

$
m(i) = \left\{
\begin{aligned}
 \frac{p_0\bmu+q_0\bnu}{p_0 + q_0} (1+o(1)) \quad \text{for}  \, i \in C_0  \, \text{and}  \, i \in H_0 \\
 \frac{q_0\bmu+p_0\bnu}{p_0 + q_0} (1+o(1)) \quad \text{for}  \, i \in C_1  \, \text{and}  \, i \in H_0 \\
 \frac{p_1\bmu+q_1\bnu}{p_1 + q_1} (1+o(1)) \quad \text{for}  \, i \in C_0  \, \text{and}  \, i \in H_1 \\
  \frac{q_1\bmu+p_1\bnu}{p_1 + q_1} (1+o(1)) \quad \text{for}  \, i \in C_1  \, \text{and}  \, i \in H_1 \\
\end{aligned}
\right.
$

